On Localizing a Camera from a Single Image

Public cameras often have limited metadata describing their attributes. A key missing attribute is the precise location of the camera, using which it is possible to precisely pinpoint the location of events seen in the camera. In this paper, we explore the following question: under what conditions is it possible to estimate the location of a camera from a single image taken by the camera? We show that, using a judicious combination of projective geometry, neural networks, and crowd-sourced annotations from human workers, it is possible to position 95% of the images in our test data set to within 12 m. This performance is two orders of magnitude better than PoseNet, a state-of-the-art neural network that, when trained on a large corpus of images in an area, can estimate the pose of a single image. Finally, we show that the camera's inferred position and intrinsic parameters can help design a number of virtual sensors, all of which are reasonably accurate.

==> abs_backup.tex <==
\section{Absolute Localization}
\label{sec:abs_loc}
In Section~\ref{sec:rel_loc}, we explained our proposed system to estimate the relative position between an Car visible on the feed of camera and the camera, denoted as $\mathbf{X}^w_{rel} = [\delta x^w, \delta y^w, \delta z^w]^T$.
In this section, we detail how we translate the relative location to the absolute location for the camera, $P_c = (lat_c, long_c)$. To this end, we first convert the relative position of the the camera and the reference points into GPS coordinate different,  $(\delta_{lat}, \delta_{long})$.

\subsection{Roadmap} 
In order to convert the relative position to the absolute position, we need to know the absolute position of the reference point.
Let us assume that we know the actual GPS location of one such reference point with image pixels location $\mathbf{X}_{rf1}^p $,  and GPS coordinate $(lat_{rf1}, long_{rf1})$. 
WLOG, let us also assume that, $\mathbf{X}^w_{rel} = [\delta x^w, \delta y^w, \delta z^w]^T$ is the relative position of camera with respect to this reference points.
Since, GPS locations does not provide height information, this reference pixel MUST correspond to a point on the ground i.e, $X^w-Y^w$ plane with $Z^w =0$. 
With this information, we know that the camera is located at some point along a circle around $(lat_{rf1}, long_{rf1})$ with a radius of $d^w_{rel} = \sqrt{(\delta x^w)^2 + (\delta y^w)^2}$. 
However, earth surface is not plane or even spherical and the latitude-longitude coordinates are the polar coordinate with respect to earth's center. There exist a range of earth model approximation~\cite{aviat} for relating latitude-longitude to distance over earth's surface that are mainly used in the context of Aviation. However, our system application region is very small compared to earth's radius and surface. Typically the region observable by the street cameras are in the orders of couple square meters. Therefore, the distance between the camera and the car is also much less than a Kilometers. For estimation of lat-long displacement over such a small regions, one can approximate the region as flat. 
Now, in a spherical earth model 90 degrees of latitude implies $\approx 10^7m$ displacement whereas the displacement for one degree of longitude is $\cos{latitude}$ times the displacement due to 1 degree of latitude.
In summary, the displacement for 1 degree latitude is $10^7/90 = 111111$ meters and for 1 degree of longitude is $111111 \times \cos(latitude)$.
With this information, we can estimate the lat-long of the camera if the bearing, $\alpha \in (-180, 180]$, from the reference point to the camera location is known. Here bearing refers to the angle between the direction from the reference point to the camera and the True North direction at that point with the positive direction towards the True East. If $\alpha$ is known, we can calculate the lat-long for the camera as,  
\begin{equation}
    \begin{split}
         lat_{c} &= lat_{rf1} + (d^w_{rel} \cdot \cos{\alpha}) / 111111)\\
         long_{c} &= long_{rf1} + (d^w_{rel} \cdot \sin{\alpha}) / (111111\cdot \cos(lat_{rf1})
    \end{split}
\end{equation}
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.7\linewidth]{images/absolute_ill.eps}
    \caption{Illustration of the Absolute Position Estimation}
    \label{fig:abs_ill}
\end{figure}
Now, one can easily use this information for three reference point and triangulate the camera location to a unique solution. But getting one reference point location accurately is tough enough. So, we further look into what can we do less than three reference points. 
To use less than three reference points, we need to estimate the value of $\alpha$.
Now the main question is, how do we estimate the $\alpha$ from the available information.
Based on the relative position estimate, $\mathbf{X}^w_{rel}$, we can estimate the angular position of the camera in $\mathbf{X}^w$. For the particular case illustrated in Fig.~\ref{fig:abs_ill}, $\phi = \arctan\frac{|\delta x^w|}{|\delta y^w|}$. Now assume that the direction of $\mathbf{X}^w$ is $\theta$ with respect to the True North and towards East. Then for this particular situation, $\alpha = 90 + \theta + \phi$. But there can be three other possible situations where the directions of $\mathbf{X}^w$ or $\mathbf{Y}^w$ or both are switched. Thus for total four four possible cases, we can get four estimates as follows.
\begin{equation}
    \begin{split}
        \alpha &= \theta + 90 + \phi \\
        \alpha &= \theta + 90 - \phi \\
        \alpha &= \theta - 90 + \phi \\
        \alpha &= \theta - 90 - \phi \\
    \end{split}
\end{equation}

Now the question is how can we get $\theta$? This is where the road in the image helps us. 
Both Google Map and OpenStreet Map API can provide us the bearing of the road. 
As long as the reference pixel is closest to the road that we consider global X axis or the reference pixel belongs to the face of a building which is facing towards the road, querying google Map API with the GPS co-ordinate of the reference point, we can get the bearing $\theta$. 
with this bearing information, the relative location information, and the absolute location of the reference point, we can narrow down the location of the camera to four candidate locations. This is illustrated in Figure~\ref{fig:fourcandidate}.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\linewidth]{images/four_candidate.png}
    \caption{Candidate Locations Based on One Reference Point; Yellow Marker is the Actual Camera Location, Red Markers are the Estimated Camera Location Candidates }
    \label{fig:fourcandidate}
\end{figure}

We can narrow it down to one location if we know two reference point locations as follows.
Let's assume that we know the GPS coordinates of the two reference reference points with pixel locations $\mathbf{X}_{rf1}^p $, $\mathbf{X}_{rf12}^p $ as $(lat_{rf1}, long_{rf1})$, $(lat_{rf2}, long_{rf2})$, respectively. 
Using the relative localization technique presented in Section~\ref{sec:rel_loc}, we can estimate the relative position of the camera with respect to both reference point as  $\mathbf{X}^w_{rel,1} = [\delta x^w_1, \delta y^w_1, \delta z^w_1]^T$ and $\mathbf{X}^w_{rel,2} = [\delta x^w_2, \delta y^w_2, \delta z^w_2]^T$. The respective ground distance to both reference points are $d^w_{1} = \sqrt{(\delta x^w_1)^2 + (\delta y^w_1)^2}$, $d^w_{2} = \sqrt{(\delta x^w_2)^2 + (\delta y^w_2)^2}$. Then using rules of geometry, the location of camera must be one of the two intersecting points of two circles centered at $(lat_{rf1}, long_{rf1})$, $(lat_{rf2}, long_{rf2})$ with radius of $d^w_{1}$ and $d^w_{2}$, respectively. Note that,  $d^w_{1}$ and $d^w_{2}$ are in meters. To get the lat-long of the points, we go through two steps.
First, we consider a co-ordinate system with the reference point 1 as $(0,0)$ point and reference point 2 as $(d,0)$ where $d$ is the distance between the reference points in meters that we can either get from the GPS coordinate and Google Map API or from the relative position estimates. In this coordinate system, the location of the intersecting points are~\cite{wolfram}:
\begin{equation}
\begin{split}
    x &= \frac{d^2 - (d^w_{2})^2 + (d^w_{1})^2}{2\cdot d} \\
    y &= \pm \sqrt{\frac{4\cdot d^2 \cdot (d^w_{1})^2 - (d^2 - (d^w_{2})^2 + (d^w_{1})^2)^2}{4\cdot d^2}}
\end{split}
\label{eqn:circleinter}
\end{equation}
However, we still have two location. To filter one location out, we check for the pixel locations of the reference point. If $x_{rf1}^p > x_{rf2}^p$ i.e, the reference point 1 is to the right of reference point 2 pixel, we take the positive value for y. Similarly, if $x_{rf1}^p < x_{rf2}^p$ we take the negative value of y. \pradipta{If $x_{rf1}^p = x_{rf2}^p$, $y$ should be 0 producing an unique result. }



Now, to convert the location to the respective latitude and longitude, we can use simple matrix transformation> A typical 2D coordinate transformation can be expressed as follows:
\begin{equation}
    \begin{split}
        x' &= p x + q y + r\\
        y' &= q x -p y + s
    \end{split}
\end{equation}
where $p, q, r, s$ are four constants and (x,y) is the location in one coordinate and (x', y') in the other. Using this equation, and the two reference point locations we can solve for $p, q, r, s$ as follows:
\begin{equation}
    \begin{bmatrix}
    lat_{rf1} \\
    long_{rf1} \\
    lat_{rf2} \\
    long_{rf2}
    \end{bmatrix} = 
    \begin{bmatrix}
     0 & 0 & 1 & 0 \\
     0 & 0 & 0 & 1 \\
     d & 0 & 1 & 0 \\
     0 & d & 0 & 1\\
     \end{bmatrix}
     \begin{bmatrix}
     p \\
     q \\
     r \\
     s
     \end{bmatrix}
\end{equation}
By solving this set of equations and combining with Eqn.~\ref{eqn:circleinter}, we can get the lat-long of the camera.   \

%	\pradipta{Another approach of using two location would be to filter out locations from the one reference point based method. Based on one reference point we can get four candidate location. Then we can use the distance to the second reference point to filter out upto 2 locations. Then we can again use the pixel locations of the reference points to filter out one location.}

So far, we discussed how CamLoc can leverage the absolute location of either one or two pixel point to output a set of possible locations for the camera. 
This leads to the following question: \emph{how do we get such points in the query image?} 
In the next two sections, we discuss two particular cases of real world scenarios where we can get such points followed by a discussion of how these points can be used in CamLoc system.
\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{images/two_corner_illustration.png}
    \caption{Illustration of the Two Corner Based Absolute Position Estimation. The top two combination of intersection are illustrated as in red and green, respectively. Then for each pair we get 2 possible locations.}
    \label{fig:twocorner}
\end{figure}
\subsection {Road Intersection}
Let us assume a very special case for the camera localization where the metadata from the public website can tell you that the camera is located near a particular road intersection. 
In addition, let us assume that we can see at least one of the corners in the query image. 
Now the questions is:  how do we use this information to get the location of camera. 
With this information, we can present the query image and a satellite view of the respective road intersection to a human annotator and ask him/her to point all the corners in both image in a Clockwise manner. 
With such annotation, we will have a ordered list of visible corner in image and ordered list of lat-long of the corner points on the intersection.
The question that is still unanswered is how can we associate the corner in the image with a particular corner on the intersection without any other information available?
WLOG, let us assume that there are four corners on the intersection as four is the most common corner count in intersections around the worlds.
Next, we will discuss four different cases.

\parab{Single Visible Corner:} If the query image contains only one corner point, it is almost impossible to associate that with a particular corner without any additional information. Thus, we can assume that it can be either of the four corners and generate 4 possible locations for each of the cases. This will lead to a solution set of 16 possible locations. 

\parab{Two Visible Corners:} If the query image contains two sequential corners, then it is possible to get 8 combination of two sequential corners (one for each direction). Using simple this information we can get 8 possible locations. However, we can get some additional information from the annotations. From the annotations and applying Eqn.~\eqref{eqn:real_landmark} we can get the position of both corners relative to the camera. Using this information, we can estimate the length of the line segment joining both corners. 
Similarly from the google map or openstreetmap we can get the actual distance between the annotated corner points. Next we simple match the distances and take the side with length closest to the estimated length.
Typically the road intersection are symmetric with opposite side having similar length. Thus, for the four corners case, the matching can return either of these similar intersection sides. Moreover, the error in the relative position estimation can also cause some error in length matching. However, best on our experiments we observed that the correct answer is always withing the top two closest segments. Thus we can take the top two corner pairs that get a set of 4 possible locations. This is illustrated in \figref{fig:twocorner}

\parab{Three Visible Corner:} If the query image contains three visible sequential corner points, we can again get 8 possible combination. However, by restricting the annotation one direction, we can narrow it to 4 possible locations which was not possible in the 2 corner case. With this, we can match the sequence of two estimated lengths with the all possible sequence of two lengths from of the real corners. In this case, ideally we should get one solution. But again due to symmetry in the road intersections as well as estimation errors, the correct combination may not be the top match but stays withing top two matches. For each combination, we can just simply apply trilateration to get one possible location. Thus we can get two possible locations for the camera.

\parab{Four Visible Corners:} Now it is also possible to be able to see all four corners in the query image. In such case, similar to three corner case, we can match the sequence of lengths. In this case too, the correct combination stays within top two due to symmetry. Thus even from four corner case, we get two possible locations.

In summary, it is not possible to narrow the Camera Location to a single location, by just using intersection proximity information. However, as shown in \secref{sec:corner_res},  one of the candidate locations is within 10 meters of the actual location with 95 percentile. This analysis is true for even larger number of corners in the intersection. The only way to narrow down to one location is if one can associate a landmark object with one of the corners. 


\subsection{Landmark Building}
Let us now consider another scenario where we can see a landmark building in the query image. Let's further assume that a human or a DNN can read the landmark sign/name to uniquely identify the building. 
% Now assuming that we know that this landmark is located within a small region such as a 5 km $\times$ 5 km regions. Now we can just search using Google Map API for the location of the landmark building. 
% However, it is quite possible to same multiple instances of similar landmark within the region of interest, for example there might be multiple Subway in that region. In this case, it become important to identify the correct one. In order to do that, we can use two types of filtering: (1) Our analysis of landmarks with same logo led to the conclusion that the buildings have different geometry, more specifically different heights. In that case we can estimate the height of the building from the images using \eqnref{} and use the height to filter out the correct landmark. (2) Another common factor separating landmarks is while some of the buildings are standalone, others are together with other landmark in a shopping complex type setting. We can leverage these information to narrow down the search space.
Once we have the correct landmark location, the next step is to position the camera relative to that landmark. 
Now the challenge is that the Geo-Tag marker for each landmark points to a random position within the landmark.
But what we see in the image is one of the face in the images. Thus it becomes challenging to associate a pixel point with the lat-long of the landmark. To this end, we explore two different approach.

\parab{Building Face Center:} In the first approach, first detect the bottom middle point of the landmark face visible in the query image.  Then we apply \eqnref{eqn:real_landmark} to estimate the camera position realtive to that point. 
Then we use Openstreet map to get the bounding box of the landmark and estimate the distance of the landmark geo-tag to each of the four faces of the bounding box and take the average, $d_\tau$. 
Now, assume the relative position of the camera wrt to the center point to be $(\delta x^w, \delta x^y)$ with distance $d^w_{rel}$.  To compensate for the distance from the face to the geotag, we update the relative location as $\delta x^w_m = \delta x^w \cdot(1 + d_\tau /d^w_{rel})$ and $\delta x^w_m= \delta x^w \cdot(1 + d_\tau /d^w_{rel}))$. We use the updated relative location to position the camera. This is illustrated in \figref{fig:lm_center}.
\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{images/landmark_illustration.png}
    \caption{Illustration Using the Landmark Building Geotag for the Absolute Position of the Camera}
    \label{fig:lm_center}
\end{figure}

\parab{Building Corners:} Similar to the road corners, we can annotate the building corners and then match it with the building polygon geometry obtained from Open Street Map. In single visible corner case the method of matching remains same as the road corner matching. But for multiple corner cases, the problem turns out to be non-trivial. The Open Street Map provides us with the exact geometry that represent every small and large face of the building. Now, in the query image, the small faces are often  not visible and hard to detect. In such case, the annotation/detection with give two corners that are not consecutive and therefore cannot be easily matched. Once would have to iterate through all possible combination of corners as a potential candidate. 

==> backup_bib <==
@inproceedings{mousavian20173d,
  title={3d bounding box estimation using deep learning and geometry},
  author={Mousavian, Arsalan and Anguelov, Dragomir and Flynn, John and Kosecka, Jana},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={7074--7082},
  year={2017}
}
@misc{earthcam,
  title = {{EarthCam}},
  howpublished = {\url{https://www.earthcam.com/}}
}
@inproceedings{schoning2009photomap,
  title={PhotoMap: using spontaneously taken images of public maps for pedestrian navigation tasks on mobile devices},
  author={Sch{\"o}ning, Johannes and Kr{\"u}ger, Antonio and Cheverst, Keith and Rohs, Michael and L{\"o}chtefeld, Markus and Taher, Faisal},
  booktitle={Proceedings of the 11th international Conference on Human-Computer interaction with Mobile Devices and Services},
  pages={14},
  year={2009},
  organization={ACM}
}
@article{wang2013intelligent,
  title={Intelligent multi-camera video surveillance: A review},
  author={Wang, Xiaogang},
  journal={Pattern recognition letters},
  volume={34},
  number={1},
  pages={3--19},
  year={2013},
  publisher={Elsevier}
}
@article{willson1994center,
author = {Willson, Reg G. and Shafer, Steven A.},
journal = {J. Opt. Soc. Am. A},
number = {11},
pages = {2946--2955},
publisher = {OSA},
title = {What is the center of the image?},
volume = {11},
month = {Nov},
year = {1994},
url = {http://josaa.osa.org/abstract.cfm?URI=josaa-11-11-2946},
doi = {10.1364/JOSAA.11.002946},
}
@inproceedings{liu2016ssd,
  title={Ssd: Single shot multibox detector},
  author={Liu, Wei and Anguelov, Dragomir and Erhan, Dumitru and Szegedy, Christian and Reed, Scott and Fu, Cheng-Yang and Berg, Alexander C},
  booktitle={European conference on computer vision},
  pages={21--37},
  year={2016},
  organization={Springer}
}
@inproceedings{orghidan2012camera,
  title={Camera calibration using two or three vanishing points},
  author={Orghidan, Radu and Salvi, Joaquim and Gordan, Mihaela and Orza, Bogdan},
  booktitle={2012 Federated Conference on Computer Science and Information Systems (FedCSIS)},
  pages={123--130},
  year={2012},
  organization={IEEE}
}
@misc{abccam,
  title = {{ABC Cams}},
  howpublished = {\url{https://abc7.com/weather/cams/}}
}
@inproceedings{tar,
 title={TAR: Enabling Fine-Grained Targeted Advertising in Retail Stores},
 author={Liu, Xiaochen and Jiang, Yurong and Jain, Puneet and Kim, Kyu-Han},
 booktitle={Proceedings of the 16th Annual International Conference on Mobile Systems, Applications, and Services},
 pages={323--336},
 year={2018},
 organization={ACM}
} 

@misc{insecam,
  title = {{InseCam}},
  howpublished = {\url{https://www.insecam.org/}}
}

@misc{aviat,
 title={\url{http://www.edwilliams.org/avform.htm#LL}},
 author={{Aviation Formulary}},
 year={2019}
 }

@misc{osm,
 title={\url{https://www.openstreetmap.org/}},
 author={{Open Street Map}},
 year={2019}
 }
 
 
@misc{7-scene,
 title={\url{https://www.microsoft.com/en-us/research/project/rgb-d-dataset-7-scenes/}},
 author={{7-Scene Dataset}},
 year={2019}
 }
 @inproceedings{lezama2014finding,
  title={Finding vanishing points via point alignments in image primal and dual domains},
  author={Lezama, Jos{\'e} and Grompone von Gioi, Rafael and Randall, Gregory and Morel, Jean-Michel},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={509--515},
  year={2014}
}
 @inproceedings{kovsecka2002video,
  title={Video compass},
  author={Ko{\v{s}}eck{\'a}, Jana and Zhang, Wei},
  booktitle={European conference on computer vision},
  pages={476--490},
  year={2002},
  organization={Springer}
}
@inproceedings{tardif2009non,
  title={Non-iterative approach for fast and accurate vanishing point detection},
  author={Tardif, Jean-Philippe},
  booktitle={2009 IEEE 12th International Conference on Computer Vision},
  pages={1250--1257},
  year={2009},
  organization={IEEE}
}
@inproceedings{wildenauer2012robust,
  title={Robust camera self-calibration from monocular images of Manhattan worlds},
  author={Wildenauer, Horst and Hanbury, Allan},
  booktitle={2012 IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2831--2838},
  year={2012},
  organization={IEEE}
}
@INPROCEEDINGS{6385802, 
author={J. {Bazin} and M. {Pollefeys}}, 
booktitle={2012 IEEE/RSJ International Conference on Intelligent Robots and Systems}, 
title={3-line RANSAC for orthogonal vanishing point detection}, 
year={2012}, 
volume={}, 
number={}, 
pages={4282-4287}, 
keywords={iterative methods;natural scenes;robot vision;sampling methods;stability;3-line RANSAC;orthogonal vanishing point detection;robotic systems;automatic control;stabilization;robot vision;urban environments;scene structure;orthogonality constraint;model estimation;minimal sampling;rotation estimation;Estimation;Real-time systems;Cameras;Clustering algorithms;Robots;Complexity theory;Google}, 
doi={10.1109/IROS.2012.6385802}, 
ISSN={2153-0866}, 
month={Oct},}

@inproceedings{barinova2010geometric,
  title={Geometric image parsing in man-made environments},
  author={Barinova, Olga and Lempitsky, Victor and Tretiak, Elena and Kohli, Pushmeet},
  booktitle={European conference on computer vision},
  pages={57--70},
  year={2010},
  organization={Springer}
}
@inproceedings{simon2016simple,
  title={A simple and effective method to detect orthogonal vanishing points in uncalibrated images of man-made environments},
  author={Simon, Gilles and Fond, Antoine and Berger, Marie-Odile},
  booktitle={Eurographics 2016},
  year={2016}
}
@misc{cambrid-data,
    title={\url{http://mi.eng.cam.ac.uk/projects/relocalisation/#dataset}},
 author={{Cambridge Dataset}},
 year={2019}
}
@misc{proj-tutorial,
    title={\url{http://www.cse.psu.edu/~rtc12/CSE486/lecture12.pdf}},
    author={{Camera Projection Tutorial}},
    year={2019}
}
@misc{vanish-tutorial,
    title={\url{http://www.cs.princeton.edu/courses/archive/fall13/cos429/lectures/11-epipolar}},
    author={{Vanishing Point Tutorial}},
    year={2019}
}
@misc{wolfram,
 title={\url{ http://mathworld.wolfram.com/Circle-CircleIntersection.html}},
 author={{Circle-Circle Intersection}},
 year={2019}
 }

@misc{klt,
 title={\url{https://en.wikipedia.org/wiki/Kanade–Lucas–Tomasi_feature_tracker}},
 author={{KLT Tracker}},
 year={2019}
 }
 
@InProceedings{Kendall_2015_ICCV,
author = {Kendall, Alex and Grimes, Matthew and Cipolla, Roberto},
title = {PoseNet: A Convolutional Network for Real-Time 6-DOF Camera Relocalization},
booktitle = {The IEEE International Conference on Computer Vision (ICCV)},
month = {December},
year = {2015}
}

@InProceedings{Laskar_2017_ICCV,
author = {Laskar, Zakaria and Melekhov, Iaroslav and Kalia, Surya and Kannala, Juho},
title = {Camera Relocalization by Computing Pairwise Relative Poses Using Convolutional Neural Network},
booktitle = {The IEEE International Conference on Computer Vision (ICCV) Workshops},
month = {Oct},
year = {2017}
} 

@INPROCEEDINGS {IM2GPS2008,
author = {J. Hays and A. A. Efros},
booktitle = {2008 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
title = {{IM2GPS: estimating geographic information from a single image}},
year = {2008},
volume = {},
issn = {},
pages = {1-8},
keywords = {},
doi = {10.1109/CVPR.2008.4587784},
url = {https://doi.ieeecomputersociety.org/10.1109/CVPR.2008.4587784},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
month = {jun}
}

@inproceedings{Iscen:2017:PPM:3078971.3079033,
 author = {Iscen, Ahmet and Tolias, Giorgos and Avrithis, Yannis and Furon, Teddy and Chum, Ond\v{r}ej},
 title = {Panorama to Panorama Matching for Location Recognition},
 booktitle = {Proceedings of the 2017 ACM on International Conference on Multimedia Retrieval},
 series = {ICMR '17},
 year = {2017},
 isbn = {978-1-4503-4701-3},
 location = {Bucharest, Romania},
 pages = {392--396},
 numpages = {5},
 url = {http://doi.acm.org/10.1145/3078971.3079033},
 doi = {10.1145/3078971.3079033},
 acmid = {3079033},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {image retrieval, location recognition},
} 

@InProceedings{Zamir2010StreeView,
author="Zamir, Amir Roshan and Shah, Mubarak",
editor="Daniilidis, Kostas and Maragos, Petros and Paragios, Nikos",
title="Accurate Image Localization Based on Google Maps Street View",
booktitle="Computer Vision -- ECCV 2010",
year="2010",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="255--268",
isbn="978-3-642-15561-1"
}

@INPROCEEDINGS{Chen2011Landmark,
author={D. M. {Chen} and G. {Baatz} and K. {Köser} and S. S. {Tsai} and R. {Vedantham} and T. {Pylvänäinen} and K. {Roimela} and X. {Chen} and J. {Bach} and M. {Pollefeys} and B. {Girod} and R. {Grzeszczuk}},
booktitle={CVPR 2011},
title={City-scale landmark identification on mobile devices},
year={2011},
volume={},
number={},
pages={737-744},
doi={10.1109/CVPR.2011.5995610},
ISSN={1063-6919},
month={June},
}

@INPROCEEDINGS{Zhang06,
author={W. {Zhang} and J. {Kosecka}},
booktitle={Third International Symposium on 3D Data Processing, Visualization, and Transmission (3DPVT'06)},
title={Image Based Localization in Urban Environments},
year={2006},
volume={},
number={},
pages={33-40},
doi={10.1109/3DPVT.2006.80},
ISSN={},
month={June},
}

@INPROCEEDINGS{GeographicalWebCam2014,
author={J. {Choe} and T. {Pramoun} and T. {Amornraksa} and Y. {Lu} and E. J. {Delp}},
booktitle={2014 Southwest Symposium on Image Analysis and Interpretation},
title={Image-based geographical location estimation using web cameras},
year={2014},
pages={73-76},
doi={10.1109/SSIAI.2014.6806032},
ISSN={},
month={April}
}

@INPROCEEDINGS {Geo2007,
author = {N. Roman and R. Pless and S. Satkin and R. Speyer and N. Jacobs},
booktitle = {2007 11th IEEE International Conference on Computer Vision},
title = {Geolocating Static Cameras},
year = {2007},
volume = {},
issn = {},
pages = {1-6},
keywords = {},
doi = {10.1109/ICCV.2007.4408995},
url = {https://doi.ieeecomputersociety.org/10.1109/ICCV.2007.4408995},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
month = {oct}
}

@INPROCEEDINGS{5711494,
author={N. {Jacobs} and K. {Miskell} and R. {Pless}},
booktitle={2011 IEEE Workshop on Applications of Computer Vision (WACV)},
title={Webcam geo-localization using aggregate light levels},
year={2011},
volume={},
number={},
pages={132-138},
keywords={computer vision;webcam geo-localization;aggregate light levels;static cameras;long-term time-lapse imagery;zenith angle;zenith-intensity relationship;outdoor webcams;Cameras;Sun;Accuracy;Calibration;Algorithm design and analysis;Optimization;Robustness},
doi={10.1109/WACV.2011.5711494},
ISSN={1550-5790},
month={Jan},
}

@inproceedings{Yan:2008:DIS:1460412.1460428,
 author = {Yan, Tingxin and Ganesan, Deepak and Manmatha, R.},
 title = {Distributed Image Search in Camera Sensor Networks},
 booktitle = {Proceedings of the 6th ACM Conference on Embedded Network Sensor Systems},
 series = {SenSys '08},
 year = {2008},
 isbn = {978-1-59593-990-6},
 location = {Raleigh, NC, USA},
 pages = {155--168},
 numpages = {14},
 url = {http://doi.acm.org/10.1145/1460412.1460428},
 doi = {10.1145/1460412.1460428},
 acmid = {1460428},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {camera sensor networks, distributed search, visterms, vocabulary tree},
} 

@inproceedings{Yan:2010:CEC:1814433.1814443,
 author = {Yan, Tingxin and Kumar, Vikas and Ganesan, Deepak},
 title = {CrowdSearch: Exploiting Crowds for Accurate Real-time Image Search on Mobile Phones},
 booktitle = {Proceedings of the 8th International Conference on Mobile Systems, Applications, and Services},
 series = {MobiSys '10},
 year = {2010},
 isbn = {978-1-60558-985-5},
 location = {San Francisco, California, USA},
 pages = {77--90},
 numpages = {14},
 url = {http://doi.acm.org/10.1145/1814433.1814443},
 doi = {10.1145/1814433.1814443},
 acmid = {1814443},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {crowdsourcing, human validation, image search, real time},
 }

@INPROCEEDINGS{ImageNet2009,
author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
booktitle={2009 IEEE Conference on Computer Vision and Pattern Recognition},
title={ImageNet: A large-scale hierarchical image database},
year={2009},
volume={},
number={},
pages={248-255},
doi={10.1109/CVPR.2009.5206848},
ISSN={1063-6919},
month={June},
}

@INPROCEEDINGS{Annotation2008,
author={A. {Sorokin} and D. {Forsyth}},
booktitle={2008 IEEE Computer Society Conference on Computer Vision and Pattern Recognition Workshops},
title={Utility data annotation with Amazon Mechanical Turk},
year={2008},
volume={},
number={},
pages={1-8},
keywords={data handling;image processing;Web services;Web sites;utility data annotation;Amazon Mechanical Turk;annotation problems;Gold;Protocols;Costs;Throughput;Humans;Quality assurance;Feedback;Computer vision;Centralized control;HTML},
doi={10.1109/CVPRW.2008.4562953},
ISSN={2160-7508},
month={June},
}

@INPROCEEDINGS{7487679,
author={A. {Kendall} and R. {Cipolla}},
booktitle={2016 IEEE International Conference on Robotics and Automation (ICRA)},
title={Modelling uncertainty in deep learning for camera relocalization},
year={2016},
volume={},
number={},
pages={4762-4769},
doi={10.1109/ICRA.2016.7487679},
ISSN={},
month={May},
}

@InProceedings{Kendall_2017_CVPR,
author = {Kendall, Alex and Cipolla, Roberto},
title = {Geometric Loss Functions for Camera Pose Regression With Deep Learning},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {July},
year = {2017}
} 

@InProceedings{Shotton_2013_CVPR,
author = {Shotton, Jamie and Glocker, Ben and Zach, Christopher and Izadi, Shahram and Criminisi, Antonio and Fitzgibbon, Andrew},
title = {{Scene Coordinate Regression Forests for Camera Relocalization in RGB-D Images}},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2013}
} 

@inproceedings{Imbriaco2019geopositioning,
author = {Imbriaco, Raffaele and Sebastian, Clint and Bondarev, Egor and de With, Peter H. N.},
title = {Towards accurate camera geopositioning by image matching},
volume = {11041},
year = {2019},
month = {March},
doi = {10.1117/12.2522999},
URL = {https://doi.org/10.1117/12.2522999},
booktitle = {Eleventh International Conference on Machine Vision (ICMV 2018)},
}


@inproceedings{li:hal-01867143,
  TITLE = {{Scene Coordinate Regression with Angle-Based Reprojection Loss for Camera Relocalization}},
  AUTHOR = {Li,  Xiaotian and Ylioinas, Juha and Verbeek, Jakob and Kannala, Juho},
  URL = {https://hal.inria.fr/hal-01867143},
  BOOKTITLE = {{ECCV 2018 - Workshop Geometry Meets Deep Learning}},
  ADDRESS = {Munich, Germany},
  PUBLISHER = {{Springer}},
  SERIES = {Lecture Notes in Computer Science},
  VOLUME = {11131},
  PAGES = {229-245},
  YEAR = {2018},
  MONTH = Sep,
  DOI = {10.1007/978-3-030-11015-4\_19},
  KEYWORDS = {camera relocalization ; scene coordinate regression ; deep neural networks},
  PDF = {https://hal.inria.fr/hal-01867143/file/li18eccvw.pdf},
  HAL_ID = {hal-01867143},
  HAL_VERSION = {v2},
}

@ARTICLE {NetVLAD2018,
author = {R. Arandjelovic and P. Gronat and A. Torii and T. Pajdla and J. Sivic},
journal = {{IEEE Transactions on Pattern Analysis \& Machine Intelligence}},
title = {{NetVLAD: CNN Architecture for Weakly Supervised Place Recognition}},
year = {2018},
volume = {40},
number = {06},
issn = {0162-8828},
pages = {1437-1451},
doi = {10.1109/TPAMI.2017.2711011},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
month = {jun}
}

@INPROCEEDINGS{VLAD2010,
author={H. {J\'{e}gou} and M. {Douze} and C. {Schmid} and P. {P\'{e}rez}},
booktitle={2010 IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
title={Aggregating local descriptors into a compact image representation},
year={2010},
volume={},
number={},
pages={3304-3311},
doi={10.1109/CVPR.2010.5540039},
ISSN={1063-6919},
month={June},
}

@InProceedings{PlaNet2016,
author="Weyand, Tobias and Kostrikov, Ilya and Philbin, James",
editor="Leibe, Bastian and Matas, Jiri and Sebe, Nicu and Welling, Max",
title="PlaNet - Photo Geolocation with Convolutional Neural Networks",
booktitle="Computer Vision -- ECCV 2016",
year="2016",
publisher="Springer International Publishing",
address="Cham",
pages="37--55",
isbn="978-3-319-46484-8",
}

@InProceedings{Cavallari2017CVPR,
author = {Cavallari, Tommaso and Golodetz, Stuart and Lord, Nicholas A. and Valentin, Julien and Di Stefano, Luigi and Torr, Philip H. S.},
title = {On-The-Fly Adaptation of Regression Forests for Online Camera Relocalisation},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {July},
year = {2017}
} 

@Article{Lowe2004,
author="Lowe, David G.",
title="Distinctive Image Features from Scale-Invariant Keypoints",
journal="International Journal of Computer Vision",
year="2004",
month="Nov",
day="01",
volume="60",
number="2",
pages="91--110",
issn="1573-1405",
doi="10.1023/B:VISI.0000029664.99615.94",
url="https://doi.org/10.1023/B:VISI.0000029664.99615.94"
}

@INPROCEEDINGS {ORB2011,
author = {G. Bradski and K. Konolige and V. Rabaud and E. Rublee},
booktitle = {2011 IEEE International Conference on Computer Vision (ICCV 2011)},
title = {{ORB: An efficient alternative to SIFT or SURF}},
year = {2011},
volume = {},
issn = {},
pages = {2564-2571},
keywords = {},
doi = {10.1109/ICCV.2011.6126544},
url = {https://doi.ieeecomputersociety.org/10.1109/ICCV.2011.6126544},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
month = {nov}
}

@INPROCEEDINGS{FREAK2012,
author={A. {Alahi} and R. {Ortiz} and P. {Vandergheynst}},
booktitle={2012 IEEE Conference on Computer Vision and Pattern Recognition},
title={FREAK: Fast Retina Keypoint},
year={2012},
volume={},
number={},
pages={510-517},
doi={10.1109/CVPR.2012.6247715},
ISSN={1063-6919},
month={June},
}

@InProceedings{Feng_2016_CVPR,
author = {Feng, Wei and Tian, Fei-Peng and Zhang, Qian and Sun, Jizhou},
title = {{6D Dynamic Camera Relocalization From Single Reference Image}},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2016}
} 

@ARTICLE {5Points2004,
author = {D. Nist{\'e}r},
journal = {IEEE Transactions on Pattern Analysis \& Machine Intelligence},
title = {An Efficient Solution to the Five-Point Relative Pose Problem},
year = {2004},
volume = {26},
number = {06},
issn = {0162-8828},
pages = {756-777},
keywords = {imaging geometry;motion;relative orientation;structure from motion;camera calibration;ego-motion estimation;scene reconstruction.},
doi = {10.1109/TPAMI.2004.17},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
month = {jun}
}

@INPROCEEDINGS{VLocNet2018,
author={A. {Valada} and N. {Radwan} and W. {Burgard}},
booktitle={2018 IEEE International Conference on Robotics and Automation (ICRA)},
title={Deep Auxiliary Learning for Visual Localization and Odometry},
year={2018},
volume={},
number={},
pages={6939-6946},
doi={10.1109/ICRA.2018.8462979},
ISSN={2577-087X},
month={May},
}

@ARTICLE{VLocNet++2018,
author={N. {Radwan} and A. {Valada} and W. {Burgard}},
journal={IEEE Robotics and Automation Letters},
title={VLocNet++: Deep Multitask Learning for Semantic Visual Localization and Odometry},
year={2018},
volume={3},
number={4},
pages={4407-4414},
doi={10.1109/LRA.2018.2869640},
ISSN={2377-3766},
month={Oct}
}

@INPROCEEDINGS{Xu2014,
author={D. {Xu} and H. {Badino} and D. {Huber}},
booktitle={2014 IEEE/RSJ International Conference on Intelligent Robots and Systems},
title={Topometric localization on a road network},
year={2014},
volume={},
number={},
pages={3448-3455},
doi={10.1109/IROS.2014.6943043},
ISSN={2153-0858},
month={Sep.},
}

@article{Fischler:1981:RSC:358669.358692,
 author = {Fischler, Martin A. and Bolles, Robert C.},
 title = {Random Sample Consensus: A Paradigm for Model Fitting with Applications to Image Analysis and Automated Cartography},
 journal = {Commun. ACM},
 issue_date = {June 1981},
 volume = {24},
 number = {6},
 month = jun,
 year = {1981},
 issn = {0001-0782},
 pages = {381--395},
 numpages = {15},
 url = {http://doi.acm.org/10.1145/358669.358692},
 doi = {10.1145/358669.358692},
 acmid = {358692},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@INPROCEEDINGS{ICT91,
author={Y. {Chen} and G. {Medioni}},
booktitle={Proceedings. 1991 IEEE International Conference on Robotics and Automation},
title={Object modeling by registration of multiple range images},
year={1991},
volume={},
number={},
pages={2724-2729 vol.3},
doi={10.1109/ROBOT.1991.132043},
ISSN={},
month={April},
}

@ARTICLE{ICT92,
author={P. J. {Besl} and N. D. {McKay}},
journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
title={A method for registration of 3-D shapes},
year={1992},
volume={14},
number={2},
pages={239-256},
doi={10.1109/34.121791},
ISSN={0162-8828},
month={Feb},
}

@inproceedings{ArmaganHRL17,
  author    = {Anil Armagan and
               Martin Hirzer and
               Peter M. Roth and
               Vincent Lepetit},
  title     = {Accurate Camera Registration in Urban Environments Using High-Level Feature Matching},
  booktitle = {British Machine Vision Conference 2017, {BMVC}},
  month = {September},
  location = {London, UK},
  year      = {2017},
}

@INPROCEEDINGS{7924572,
author={N. {Bhowmik} and and V. {Gouet-Brunet} and B. {Soheilian}},
booktitle={2017 Joint Urban Remote Sensing Event (JURSE)},
title={Cross-domain image localization by adaptive feature fusion},
year={2017},
volume={},
number={},
pages={1-4},
% doi={10.1109/JURSE.2017.7924572},
% ISSN={},
month={March},
}

@INPROCEEDINGS{7410667,
author={B. {Zeisl} and T. {Sattler} and M. {Pollefeys}},
booktitle={2015 IEEE International Conference on Computer Vision (ICCV)},
title={Camera Pose Voting for Large-Scale Image-Based Localization},
year={2015},
volume={},
number={},
pages={2704-2712},
% doi={10.1109/ICCV.2015.310},
% ISSN={2380-7504},
month={Dec},
}

 @InProceedings{Bansal_2014_CVPR,
author = {Bansal, Mayank and Daniilidis, Kostas},
title = {Geometric Urban Geo-Localization},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2014}
}

@INPROCEEDINGS{storefronts2015,
author={Y. {Movshovitz-Attias} and Q. {Yu} and M. C. {Stumpe} and V. {Shet} and S. {Arnoud} and L. {Yatziv}},
booktitle={2015 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
title={Ontological supervision for fine grained classification of Street View storefronts},
year={2015},
volume={},
number={},
pages={1693-1702},
% doi={10.1109/CVPR.2015.7298778},
% ISSN={1063-6919},
month={June},
}

@ARTICLE{Vanishing2003,
author={A. {Almansa} and A. {Desolneux} and S. {Vamech}},
journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
title={Vanishing point detection without any a priori information},
year={2003},
volume={25},
number={4},
pages={502-507},
% doi={10.1109/TPAMI.2003.1190575},
% ISSN={0162-8828},
month={April},
}

@ARTICLE{Stein2018Sport,
author={M. {Stein} and H. {Janetzko} and A. {Lamprecht} and T. {Breitkreutz} and P. {Zimmermann} and B. {Goldlücke} and T. {Schreck} and G. {Andrienko} and M. {Grossniklaus} and D. A. {Keim}},
journal={IEEE Transactions on Visualization and Computer Graphics},
title={Bring It to the Pitch: Combining Video and Movement Data to Enhance Team Sport Analysis},
year={2018},
volume={24},
number={1},
pages={13-22},
% doi={10.1109/TVCG.2017.2745181},
% ISSN={1077-2626},
month={Jan},
}

@inproceedings{Halvorsen:2013:BIS:2483977.2483982,
 author = {Halvorsen, P{\aa}l and S{\ae}grov, Simen and Mortensen, Asgeir and Kristensen, David K. C. and Eichhorn, Alexander and Stenhaug, Magnus and Dahl, Stian and Stensland, H{\aa}kon Kvale and Gaddam, Vamsidhar Reddy and Griwodz, Carsten and Johansen, Dag},
 title = {Bagadus: An Integrated System for Arena Sports Analytics: A Soccer Case Study},
 booktitle = {Proceedings of the 4th ACM Multimedia Systems Conference},
 series = {MMSys '13},
 year = {2013},
%  isbn = {978-1-4503-1894-5},
%  location = {Oslo, Norway},
 pages = {48--59},
 numpages = {12},
%  url = {http://doi.acm.org/10.1145/2483977.2483982},
%  doi = {10.1145/2483977.2483982},
%  acmid = {2483982},
%  publisher = {ACM},
%  address = {New York, NY, USA},
%  keywords = {camera array, sensor tracking, soccer system, sport analytics, system integration, video annotation},
} 
@inproceedings{cula2001compact,
  title={Compact representation of bidirectional texture functions},
  author={Cula, Oana G and Dana, Kristin J},
  booktitle={Proceedings of the 2001 IEEE Computer Society Conference on Computer Vision and Pattern Recognition. CVPR 2001},
  volume={1},
  pages={I--I},
  year={2001},
  organization={IEEE}
}

@inproceedings{sattler2015hyperpoints,
  title={Hyperpoints and fine vocabularies for large-scale location recognition},
  author={Sattler, Torsten and Havlena, Michal and Radenovic, Filip and Schindler, Konrad and Pollefeys, Marc},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={2102--2110},
  year={2015}
}
@article{koenderink1991affine,
  title={Affine structure from motion},
  author={Koenderink, Jan J and Van Doorn, Andrea J},
  journal={JOSA A},
  volume={8},
  number={2},
  pages={377--385},
  year={1991},
  publisher={Optical Society of America}
}
@article{prusak2008pose,
  title={Pose estimation and map building with a time-of-flight-camera for robot navigation},
  author={Prusak, A and Melnychuk, O and Roth, H and Schiller, Ingo and Koch, Reinhard},
  journal={International Journal of Intelligent Systems Technologies and Applications},
  volume={5},
  number={3/4},
  pages={355--364},
  year={2008},
  publisher={Inderscience Publishers}
}

@article{sattler2017efficient,
  title={Efficient \& effective prioritized matching for large-scale image-based localization},
  author={Sattler, Torsten and Leibe, Bastian and Kobbelt, Leif},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={39},
  number={9},
  pages={1744--1756},
  year={2017},
  publisher={IEEE}
}
@inproceedings{valentin2015exploiting,
  title={Exploiting uncertainty in regression forests for accurate camera relocalization},
  author={Valentin, Julien and Nie{\ss}ner, Matthias and Shotton, Jamie and Fitzgibbon, Andrew and Izadi, Shahram and Torr, Philip HS},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={4400--4408},
  year={2015}
}
@inproceedings{philbin2007object,
  title={Object retrieval with large vocabularies and fast spatial matching},
  author={Philbin, James and Chum, Ondrej and Isard, Michael and Sivic, Josef and Zisserman, Andrew},
  booktitle={2007 IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1--8},
  year={2007},
  organization={IEEE}
}
@INPROCEEDINGS{tennis2013,
author={R. M. {Nieto} and J. M. M. {S\'{a}nchez}},
booktitle={2013 10th IEEE International Conference on Advanced Video and Signal Based Surveillance},
title={An automatic system for sports analytics in multi-camera tennis videos},
year={2013},
volume={},
number={},
pages={438-442},
doi={10.1109/AVSS.2013.6636679},
ISSN={},
month={Aug},
}
@book{prince2012computer,
  title={Computer vision: models, learning, and inference},
  author={Prince, Simon JD},
  year={2012},
  publisher={Cambridge University Press}
}
@article{Satyam,
  author    = {Hang Qiu and
               Krishna Chintalapudi and
               Ramesh Govindan},
  title     = {Satyam: Democratizing Groundtruth for Machine Vision},
  journal   = {CoRR},
  volume    = {abs/1811.03621},
  year      = {2018},
  url       = {http://arxiv.org/abs/1811.03621},
  archivePrefix = {arXiv},
%   eprint    = {1811.03621},
%   timestamp = {Fri, 23 Nov 2018 12:43:51 +0100},
%   biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1811-03621},
%   bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{rother2002new,
  title={A new approach to vanishing point detection in architectural environments},
  author={Rother, Carsten},
  journal={Image and Vision Computing},
  volume={20},
  number={9-10},
  pages={647--655},
  year={2002},
  publisher={Elsevier}
}

@inproceedings{carloc,
 author = {Jiang, Yurong and Qiu, Hang and McCartney, Matthew and Sukhatme, Gaurav and Gruteser, Marco and Bai, Fan and Grimm, Donald and Govindan, Ramesh},
 title = {CARLOC: Precise Positioning of Automobiles},
 booktitle = {Proceedings of the 13th ACM Conference on Embedded Networked Sensor Systems},
 series = {SenSys '15},
 year = {2015},
%  isbn = {978-1-4503-3631-4},
 location = {Seoul, South Korea},
 pages = {253--265},
 numpages = {13},
%  url = {http://doi.acm.org/10.1145/2809695.2809725},
%  doi = {10.1145/2809695.2809725},
%  acmid = {2809725},
%  publisher = {ACM},
%  address = {New York, NY, USA},
%  keywords = {GPS, accuracy, map},
} 

==> camloc_system_relative.tex <==
\section{CamLoc System}
\label{sec:camloc}
In this section, we details our implementation of the camera localization  system instance, that we refer to as CamLoc, which employs the concepts discussed in \secref{sec:rel_loc} and \secref{sec:abs_loc}. The CamLoc system has 6 component as illustrated in \figref{fig:camloc_system}: (1) Car Detection and Dimension Estimation (2) Car Axis Annotation, (3) Orthogonal Vanishing Point Detection, (4) Relative Position Estimation, (5) Pixel to GPS Mapping, (6) Absolute Location Estimation. Next, we briefly explain each of the modules along with how they interconnect. The input to the system is an image sampled from the camera feed.



\parab{Car Detection and Dimension Estimation.}
This is the very first module in the system that input the query image and outputs the 2D bounding of the most-visible along with its three dimensions (L, H, W). This module perform two sequential tasks: \emph{Car Detection and Car Dimension estimation.}
For the car detection, we employ a very well known pre-trained object detection tool  called SSD~\cite{liu2016ssd}~\footnote{\url{https://github.com/balancap/SSD-Tensorflow}}. For the car dimension estimation, we use a standard predetermined dimensions of a Sedan (detailed in \secref{sec:rel_loc}).  
We also have a provision of using a pre-trained DNN for dimension estimation.  For the purpose of comparative experiments presented in \secref{sec:experiment}, we will refer to the system with DNN as \emph{``CamLoc-NN''} to differentiate from the normal implementation of CamLoc.

\begin{figure*}
    \centering
   	\includegraphics[width=0.8\linewidth]{images/rel_system.png}
    	\caption{CamLoc System Illustration}
    \label{fig:camloc_system}
\end{figure*}

\parab{Car Axis Annotation.} This module of CamLoc system inputs the query image along with the bounding box of the selected car and outputs the pixel points corresponding to the World Origin and three dimensions of the car as illustrated in Fig.~\ref{fig:caraxis}. 
To this end, we employ an image
annotation crowd-sourcing service~\cite{Satyam} for Amazon Mechanical Turk platform (mentioned in \secref{sec:annotations}). 


\parab{Orthogonal Vanishing Point Detection.}
This module outputs the three orthogonal vanishing points using the Amazon Mechanical Turk based annotations detailed in \secref{sec:annotations}. For the purpose of comparison in \secref{sec:experiment}, we also have a provision of using automated edge detection based RANSAC method for three orthogonal vanishing point detection~\cite{Fischler:1981:RSC:358669.358692}.
To differentiate from the default implementation of CamLoc, we will refer the the CamLoc system with automated vanishing point detection as \emph{``CamLoc-Auto.''}

\parab{Relative Position Estimation.}
This module of CamLoc gathers all three types of information i.e., car dimensions, car axis points, and three orthogonal vanishing points to estimate the camera's intrinsic and extrinsic parameters using the techniques detailed in \secref{sec:rel_loc}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "camloc"
%%% End:


\parab{Pixel to GPS Mapping.}
To get the pixel to GPS mapping in CamLoc, we rely fully on human turkers/annotators. Human turkers are asked to perform three types of annotations: (1) Exact mapping of two pixel points to the GPS coordinate by showing them the query image and the a small region around the camera's true location, (2) Annotations of the visible corners in the image and the corners of the known intersection in Clockwise order for the known road intersection scenario detailed in \secref{sec:pixtogps}, and (3) Annotation of landmark midpoint and corners for the known landmark scenario detailed in \secref{sec:pixtogps}.

\parab{Absolute Location Estimation.}
This module of CamLoc system employes the concept discussed in \secref{sec:abs_loc} to output a set of location hypothesis based on the amount of information available. 

We also have an instance of CamLoc where all the annotations are done by a single experience human annotator to test CamLoc system's performance with a single good annotation. We will denote this instance of CamLoc as \emph{``CamLoc-Expert-Anno''}.

==> misc.tex <==
\section{Miscellaneous}
In this section, we details some additional contributions to the community. This includes a simplified ground truth annotation tools. ...

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "camloc"
%%% End:

==> problem.tex <==
\section{Problem Formulation}

%\ramesh{Move this text to another file to reduce clutter in the top-level file?}

In this paper, we are interested in the problem of localizing public street-facing web-cameras and estimate their intrinsic and extrinsic matrix parameters based on the available information as well as the accessible camera feeds. 
Let us first assume that the unknown GPS coordinate of the camera is $(lat_{c}, long_{c})$ and the camera is mounted at a  height of $h$.
Let us further assume that we know the actual GPS location of two image pixels corresponding to $\mathbf{X}_{rf1}^p $, $\mathbf{X}_{rf2}^p $ as $(lat_{rf1}, long_{rf1})$ and $(lat_{rf2}, long_{rf2})$ respectively. We will refer such points as the \emph{``Reference Points''}.
We further assume that the camera is a street facing camera with active traffic. 
Our overall goal is to estimate the GPS coordinate of the camera as well as the intrinsic and extrinsic parameters of the camera, by leveraging the accessible camera feed and other publicly available datasets and APIs. 

This objective translates to three different sequential sub-objectives:

(1) Estimate the relative position of the the camera and the reference points in terms of meters i.e,  $\mathbf{X}^w_{rel} = (\delta x^w, \delta y^w, \delta z^w)$ in the world coordinate system, $\mathcal{R}^w$. .

(2) Convert the relative position of the the camera and the reference points into GPS coordinate different,  $(\delta_{lat}, \delta_{long})$.

(3) Get two of more reference points in order to estimate the real locations. 

